Extraction of Airways using Graph Neural Networks

We present extraction of tree structures, such as airways, from image data as a graph refinement task. To this end, we propose a graph auto-encoder model that uses an encoder based on graph neural networks (GNNs) to learn embeddings from input node features and a decoder to predict connections between nodes. Performance of the GNN model is compared with mean-field networks in their ability to extract airways from 3D chest CT scans.

==> references.tex <==
@article{dijkstra1959note,
  title={A note on two problems in connexion with graphs},
  author={Dijkstra, Edsger W},
  journal={Numerische mathematik},
  volume={1},
  number={1},
  pages={269--271},
  year={1959},
  publisher={Springer}
}


@article{reid1979algorithm,
  title={An algorithm for tracking multiple targets},
  author={Reid, Donald},
  journal={IEEE transactions on Automatic Control},
  volume={24},
  number={6},
  pages={843--854},
  year={1979},
  publisher={IEEE}
}

@article{li2015gated,
  title={Gated graph sequence neural networks},
  author={Li, Yujia and Tarlow, Daniel and Brockschmidt, Marc and Zemel, Richard},
  journal={arXiv preprint arXiv:1511.05493},
  year={2015}
}

@article{scarselli2009graph,
  title={The graph neural network model},
  author={Scarselli, Franco and Gori, Marco and Tsoi, Ah Chung and Hagenbuchner, Markus and Monfardini, Gabriele},
  journal={IEEE Transactions on Neural Networks},
  volume={20},
  number={1},
  pages={61--80},
  year={2009},
  publisher={IEEE}
}

@article{lee1994building,
  title={Building skeleton models via 3-D medial surface axis thinning algorithms},
  author={Lee, Ta-Chih and Kashyap, Rangasami L and Chu, Chong-Nam},
  journal={CVGIP: Graphical Models and Image Processing},
  volume={56},
  number={6},
  pages={462--478},
  year={1994},
  publisher={Elsevier}
}

@article{li2014mean,
  title={Mean-Field Networks},
  author={Li, Yujia and Zemel, Richard},
  journal={arXiv preprint arXiv:1410.5884},
  year={2014}
}


@inproceedings{mori1996recognition,
  title={Recognition of bronchus in three-dimensional X-ray CT images with applications to virtualized bronchoscopy system},
  author={Mori, Kensaku and Hasegawa, Jun-ichi and Toriwaki, Jun-ichiro and Anno, Hirofumi and Katada, Kazuhiro},
  booktitle={Pattern Recognition, 1996., Proceedings of the 13th International Conference on},
  volume={3},
  pages={528--532},
  year={1996},
  organization={IEEE}
}

@book{chung1997spectral,
  title={Spectral graph theory},
  author={Chung, Fan RK},
  number={92},
  year={1997},
  publisher={American Mathematical Soc.}
}

@inproceedings{frangi1998multiscale,
  title={Multiscale vessel enhancement filtering},
  author={Frangi, Alejandro F and Niessen, Wiro J and Vincken, Koen L and Viergever, Max A},
  booktitle={International Conference on Medical Image Computing and Computer-Assisted Intervention},
  pages={130--137},
  year={1998},
  organization={Springer}
}

@article{nakano2000computed,
  title={Computed tomographic measurements of airway dimensions and emphysema in smokers: correlation with lung function},
  author={Nakano, Yasutaka and Muro, Shigeo and Sakai, Hiroaki and Hirai, Toyohiro and Chin, Kazuo and Tsukino, Mitsuhiro and Nishimura, Koichi and Itoh, Harumi and Par{\'e}, Peter D and Hogg, James C and others},
  journal={American journal of respiratory and critical care medicine},
  volume={162},
  number={3},
  pages={1102--1108},
  year={2000},
  publisher={Am Thoracic Soc}
}


@phdthesis{lin2001enhancement,
  title={Enhancement, detection, and visualization of 3D volume data},
  author={Lin, Qingfen},
  year={2001},
  school={Link{\"o}ping University, Department of Electrical Engineering}
}

@article{blackman2004multiple,
  title={Multiple hypothesis tracking for multiple target tracking},
  author={Blackman, Samuel S},
  journal={IEEE Aerospace and Electronic Systems Magazine},
  volume={19},
  number={1},
  pages={5--18},
  year={2004},
  publisher={IEEE}
}
@article{wink2004multiscale,
  title={Multiscale vessel tracking},
  author={Wink, Onno and Niessen, Wiro J and Viergever, Max A},
  journal={IEEE Transactions on Medical Imaging},
  volume={23},
  number={1},
  pages={130--133},
  year={2004},
  publisher={IEEE}
}


@inproceedings{florin2005particle,
  title={Particle filters, a quasi-monte carlo solution for segmentation of coronaries},
  author={Florin, Charles and Paragios, Nikos and Williams, Jim},
  booktitle={International Conference on Medical Image Computing and Computer-Assisted Intervention},
  pages={246--253},
  year={2005},
  organization={Springer}
}
@article{hasegawa2006airflow,
  title={Airflow limitation and airway dimensions in chronic obstructive pulmonary disease},
  author={Hasegawa, Masaru and Nasuhara, Yasuyuki and Onodera, Yuya and Makita, Hironi and Nagai, Katsura and Fuke, Satoshi and Ito, Yoko and Betsuyaku, Tomoko and Nishimura, Masaharu},
  journal={American journal of respiratory and critical care medicine},
  volume={173},
  number={12},
  pages={1309--1315},
  year={2006},
  publisher={Am Thoracic Soc}
}

@inproceedings{schlichtkrull2017modeling,
  title={Modeling Relational Data with Graph Convolutional Networks},
  author={Schlichtkrull, Michael and Kipf, Thomas N and Bloem, Peter and Berg, Rianne van den and Titov, Ivan and Welling, Max},
  booktitle={ESWC},
  year={2018}
}


@inproceedings{lacoste2006coronary,
  title={Coronary tree extraction from X-ray angiograms using marked point processes},
  author={Lacoste, Caroline and Finet, G{\'e}rard and Magnin, Isabelle E},
  booktitle={Biomedical Imaging: Nano to Macro, 2006. 3rd IEEE International Symposium on},
  pages={157--160},
  year={2006},
  organization={IEEE}
}

@inproceedings{yedidya2008tracking,
  title={Tracking of blood vessels in retinal images using Kalman filter},
  author={Yedidya, Tamir and Hartley, Richard},
  booktitle={Computing: Techniques and Applications, 2008. DICTA'08. Digital Image},
  pages={52--58},
  year={2008},
  organization={IEEE}
}


@article{metz20083d,
  title={3D segmentation in the clinic: A grand challenge II-coronary artery tracking},
  author={Metz, Coert and Schaap, Michiel and van Walsum, Theo and van der Giessen, Alina and Weustink, Annick and Mollet, Nico and Krestin, Gabriel and Niessen, Wiro},
  journal={Insight Journal},
  volume={1},
  number={5},
  pages={6},
  year={2008}
}

@inproceedings{friman2008coronary,
  title={Coronary centerline extraction using multiple hypothesis tracking and minimal paths},
  author={Friman, Ola and K{\"u}hnel, C and Peitgen, Heinz-Otto},
  booktitle={Proc MICCAI},
  volume={42},
  year={2008}
}
@article{rosamond2008heart,
  title={Heart disease and stroke statistics—2008 update},
  author={Rosamond, Wayne and Flegal, Katherine and Furie, Karen and Go, Alan and Greenlund, Kurt and Haase, Nancy and Hailpern, Susan M and Ho, Michael and Howard, Virginia and Kissela, Bret and others},
  journal={Circulation},
  volume={117},
  number={4},
  pages={e25--e146},
  year={2008},
  publisher={Am Heart Assoc}
}
@article{bauer2008edge,
  title={Edge based tube detection for coronary artery centerline extraction},
  author={Bauer, Christian and Bischof, Horst},
  journal={The Insight Journal},
  year={2008}
}
@article{lesage2009review,
  title={A review of 3D vessel lumen segmentation techniques: Models, features and extraction schemes},
  author={Lesage, David and Angelini, Elsa D and Bloch, Isabelle and Funka-Lea, Gareth},
  journal={Medical image analysis},
  volume={13},
  number={6},
  pages={819--845},
  year={2009},
  publisher={Elsevier}
}

@article{schaap2009standardized,
  title={Standardized evaluation methodology and reference database for evaluating coronary artery centerline extraction algorithms},
  author={Schaap, Michiel and Metz, Coert T and van Walsum, Theo and van der Giessen, Alina G and Weustink, Annick C and Mollet, Nico R and Bauer, Christian and Bogunovi{\'c}, Hrvoje and Castro, Carlos and Deng, Xiang and others},
  journal={Medical image analysis},
  volume={13},
  number={5},
  pages={701--714},
  year={2009},
  publisher={Elsevier}
}

@article{pedersen2009danish,
  title={The Danish randomized lung cancer {CT} screening trial—overall design and results of the prevalence round},
  author={Pedersen, Jesper H and Ashraf, Haseem and Dirksen, and et.al},
  journal={Journal of Thoracic Oncology},
  volume={4},
  number={5},
  year={2009},
  publisher={Elsevier}
}

@inproceedings{lo2009airway,
  title={Airway tree extraction with locally optimal paths},
  author={Lo, Pechin and Sporring, Jon and Pedersen, Jesper and et.al},
  booktitle={International Conference on Medical Image Computing and Computer-Assisted Intervention},
  year={2009},
  }

@inproceedings{wang2009new,
  title={A new localized superpixel Markov random field for image segmentation},
  author={Wang, XiaoFeng and Zhang, Xiao-Ping},
  booktitle={Multimedia and Expo, 2009. ICME 2009. IEEE International Conference on},
  pages={642--645},
  year={2009},
  organization={IEEE}
}
@article{friman2010multiple,
  title={Multiple hypothesis template tracking of small 3D vessel structures},
  author={Friman, Ola and Hindennach, Milo and K{\"u}hnel, Caroline and Peitgen, Heinz-Otto},
  journal={Medical image analysis},
  volume={14},
  number={2},
  pages={160--171},
  year={2010},
  publisher={Elsevier}
}

@article{lo2010vessel,
  title={Vessel-guided airway tree segmentation: A voxel classification approach},
  author={Lo, Pechin and Sporring, Jon and Ashraf, Haseem and Pedersen, Jesper JH and de Bruijne, Marleen},
  journal={Medical image analysis},
  volume={14},
  number={4},
  pages={527--538},
  year={2010},
  publisher={Elsevier}
}

@article{yang2012automatic,
  title={Automatic centerline extraction of coronary arteries in coronary computed tomographic angiography},
  author={Yang, Guanyu and Kitslaar, Pieter and Frenay, Michel and Broersen, Alexander and Boogers, Mark J and Bax, Jeroen J and Reiber, Johan HC and Dijkstra, Jouke},
  journal={The international journal of cardiovascular imaging},
  volume={28},
  number={4},
  pages={921--933},
  year={2012},
  publisher={Springer}
}

@inproceedings{turetken2012automated,
  title={Automated reconstruction of tree structures using path classifiers and mixed integer programming},
  author={T{\"u}retken, Engin and Benmansour, Fethallah and Fua, Pascal},
  booktitle={Computer Vision and Pattern Recognition (CVPR), 2012 IEEE Conference on},
  pages={566--573},
  year={2012},
  organization={IEEE}
}

@article{lo2012extraction,
  title={Extraction of airways from CT (EXACT'09)},
  author={Lo, Pechin and Van Ginneken, Bram and Reinhardt, Joseph M and Yavarna, Tarunashree and De Jong, Pim A and Irving, Benjamin and Fetita, Catalin and Ortner, Margarete and Pinho, R{\^o}mulo and Sijbers, Jan and others},
  journal={IEEE Transactions on Medical Imaging},
  volume={31},
  number={11},
  pages={2093--2107},
  year={2012},
  publisher={IEEE}
}

@article{wang2013markov,
  title={Markov random field modeling, inference \& learning in computer vision \& image understanding: A survey},
  author={Wang, Chaohui and Komodakis, Nikos and Paragios, Nikos},
  journal={Computer Vision and Image Understanding},
  volume={117},
  number={11},
  pages={1610--1627},
  year={2013},
  publisher={Elsevier}
}

@inproceedings{zheng2013robust,
  title={Robust and accurate coronary artery centerline extraction in CTA by combining model-driven and data-driven approaches},
  author={Zheng, Yefeng and Tek, Huseyin and Funka-Lea, Gareth},
  booktitle={International Conference on Medical Image Computing and Computer-Assisted Intervention},
  pages={74--81},
  year={2013},
  organization={Springer}
}

@article{cetin2013vessel,
  title={Vessel tractography using an intensity based tensor model with branch detection},
  author={Cetin, Suheyla and Demir, Ali and Yezzi, Anthony and Degertekin, Muzaffer and Unal, Gozde},
  journal={IEEE transactions on medical imaging},
  volume={32},
  number={2},
  pages={348--363},
  year={2013},
  publisher={IEEE}
}

@inproceedings{orlando2014learning,
  title={Learning fully-connected CRFs for blood vessel segmentation in retinal images},
  author={Orlando, Jos{\'e} Ignacio and Blaschko, Matthew},
  booktitle={International Conference on Medical Image Computing and Computer-Assisted Intervention},
  pages={634--641},
  year={2014},
  organization={Springer}
}


@article{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}
@article{cetin2015higher,
  title={A higher-order tensor vessel tractography for segmentation of vascular structures},
  author={Cetin, Suheyla and Unal, Gozde},
  journal={IEEE transactions on medical imaging},
  volume={34},
  number={10},
  pages={2172--2185},
  year={2015},
  publisher={IEEE}
}
@inproceedings{li2015superpixel,
  title={Superpixel segmentation using linear spectral clustering},
  author={Li, Zhengqin and Chen, Jiansheng},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={1356--1363},
  year={2015}
}

@inproceedings{kipf2016variational,
  title={Variational graph auto-encoders},
  author={Kipf, Thomas N and Welling, Max},
  booktitle={NIPS Bayesian Deep Learning Workshop},
  year={2016}
}

@inproceedings{milletari2016v,
  title={V-net: Fully convolutional neural networks for volumetric medical image segmentation},
  author={Milletari, Fausto and Navab, Nassir and Ahmadi, Seyed-Ahmad},
  booktitle={3D Vision (3DV), 2016 Fourth International Conference on},
  pages={565--571},
  year={2016},
  organization={IEEE}
}


@inproceedings{kipf2016semi,
  title={Semi-supervised classification with graph convolutional networks},
  author={Kipf, Thomas N and Welling, Max},
  booktitle={ICLR},
  year={2017}
}


@incollection{selvan2016extraction,
  title={Extraction of airway trees using multiple hypothesis tracking and template matching},
  author={Selvan, Raghavendra and Petersen, Jens and Pedersen, Jesper H and de Bruijne, Marleen},  
  booktitle={The Sixth International Workshop on Pulmonary Image Analysis},
  isbn={9781537038582},
  year={2016},
  publisher={CreateSpace Independent Publishing Platform}
}

@article{gilmer2017neural,
  title={Neural message passing for quantum chemistry},
  author={Gilmer, Justin and Schoenholz, Samuel S and Riley, Patrick F and Vinyals, Oriol and Dahl, George E},
  journal={arXiv preprint arXiv:1704.01212},
  year={2017}
}

@article{kuo2017diagnosis,
  title={Diagnosis of bronchiectasis and airway wall thickening in children with cystic fibrosis: Objective airway-artery quantification},
  author={Kuo, Wieying and de Bruijne, Marleen and Petersen, Jens and Nasserinejad, Kazem and Ozturk, Hadiye and Chen, Yong and Perez-Rovira, Adria and Tiddens, Harm AWM},
  journal={European Radiology},
  pages={1--10},
  year={2017},
  publisher={Springer}
}

@incollection{selvan2017extraction,
  title={Extraction of Airways with Probabilistic State-space Models and {B}ayesian Smoothing},
  author={Selvan, Raghavendra and Petersen, Jens and Pedersen, Jesper H and et.al},
  booktitle={Graphs in Biomedical Image Analysis},
  year={2017},
  }
@inproceedings{meng2017tracking,
  title={Tracking and Segmentation of the Airways in Chest CT Using a Fully Convolutional Network},
  author={Meng, Qier and Roth, Holger R and Kitasaka, Takayuki and Oda, Masahiro and Ueno, Junji and Mori, Kensaku},
  booktitle={International Conference on Medical Image Computing and Computer-Assisted Intervention},
  pages={198--207},
  year={2017},
  organization={Springer}
}

@article{berg2017graph,
  title={Graph Convolutional Matrix Completion},
  author={van den Berg, Rianne and Kipf, Thomas N and Welling, Max},
  journal={arXiv preprint arXiv:1706.02263},
  year={2017}
}

@article{ktena2017metric,
  title={Metric learning with spectral graph convolutions on brain connectivity networks},
  author={Ktena, Sofia Ira and Parisot, Sarah and Ferrante, Enzo and Rajchl, Martin and Lee, Matthew and Glocker, Ben and Rueckert, Daniel},
  journal={NeuroImage},
  year={2017},
  publisher={Elsevier}
}

@article{selvan2018mean,
  title={Mean Field Network based Graph Refinement with application to Airway Tree Extraction},
  author={Selvan, Raghavendra and Welling, Max and Petersen, Jens and Pedersen, Jesper H and de Bruijne, Marleen},
  journal={arXiv:1804.03348},
  year={2018}
}

@article{yoon2018inference,
  title={Inference in Probabilistic Graphical Models by Graph Neural Networks},
  author={Yoon, KiJung and Liao, Renjie and Xiong, Yuwen and Zhang, Lisa and et.al},
  journal={arXiv preprint arXiv:1803.07710},
  year={2018}
}
